Analyzing TCP Throughput Stability and Predictability with Implications for Adaptive Video Streaming

Recent work suggests that TCP throughput stability and predictability within a video viewing session can inform the design of better video bitrate adaptation algorithms. Despite a rich tradition of Internet measurement, however, our understanding of throughput stability and predictability is quite limited. To bridge this gap, we present a measurement study of throughput stability using a large-scale dataset from a video service provider. Drawing on this analysis, we propose a simple-but-effective prediction mechanism based on a hidden Markov model and demonstrate that it outperforms other approaches. We also show the practical implications in improving the user experience of adaptive video streaming.

==> macros.tex <==
\newcommand{\tool}{iCache\xspace}

\newcommand{\minimize}{Minimze}
\newcommand{\totalLatency}{TotalLatency}
\newcommand{\epochLatency}{EpochLatency}
\newcommand{\epochRequests}{EpochRequests}
\newcommand{\reqsServed}{ReqsServed}
\newcommand{\serve}{Serve}
\newcommand{\router}{r}
\newcommand{\epoch}{t}
\newcommand{\user}{u}
\newcommand{\object}{o}
\newcommand{\performance}{L}
\newcommand{\cacheSize}{B}
\newcommand{\hasObject}{D}
\newcommand{\hasCache}{E}
\newcommand{\averageQueryDelay}{l}
\newcommand{\interest}{I}
\newcommand{\fixedCost}{C_{fixed}}
\newcommand{\variableCost}{C_{var}}
\newcommand{\unitRevenue}{UnitRevenue}
\newcommand{\budget}{Budget}
\newcommand{\cached}{Cached}
\newcommand{\uncached}{Uncached}

%old stuff
\newcommand{\Name}{FlowTags\xspace}
\newcommand{\NameCaps}{{FLOWTAGS}}
\newcommand{\NameTable}{TagsTable\xspace}

\newcommand{\DPG}{DPG\xspace}
\newcommand{\DPGs}{DPGs\xspace}
\newcommand{\PhysDPG}{DPGImpl\xspace}
\newcommand{\Graph}{G}



\newcommand{\OriginBind}{\textsc{OriginBinding}\xspace}
\newcommand{\PathBind}{\textsc{PathsFollowPolicy}\xspace}
\newcommand{\HiLevelNames}{\textsc{HighLevelNames}\xspace}

\newcommand{\TagVar}{\ensuremath{T}}
\newcommand{\TagVarIndex}{\ensuremath{t}}

\newcommand{\rqst}{\ensuremath{\mathit{rqst}}}
\newcommand{\Switch}{\ensuremath{\mathit{Switch}}}
\newcommand{\TagUniverse}{\ensuremath{\mathit{AllTags}}}
\newcommand{\ActiveTags}{\ensuremath{\mathit{ActiveT}}}
\newcommand{\ActiveTagsTable}{\ensuremath{\mathit{ActiveTagsMap}}}
\newcommand{\SwitchInterface}{\ensuremath{\mathit{InPort}}}
\newcommand{\SwitchOutInterface}{\ensuremath{\mathit{OutPort}}}
\newcommand{\switchintindex}{\ensuremath{\mathit{s}}}
\newcommand{\Path}{\ensuremath{\mathit{Path}}}


\newcommand{\OrigFiveTuple}{\ensuremath{\mathit{OrigHdr}}}
\newcommand{\FlowHdr}{\ensuremath{\mathit{FlowMatch}}}
\newcommand{\NodeContext}{\ensuremath{\mathit{C}}}
\newcommand{\EdgeContext}{\ensuremath{\mathit{EC}}}
\newcommand{\ContextIndex}{\ensuremath{j}}

\newcommand{\Tag}{tag\xspace}


\newcommand{\totalTags}{R\xspace}
\newcommand{\tagQueue}{Q}
\newcommand{\qHead}{head}
\newcommand{\TagEnc}{TagEnc\xspace}
\newcommand{\Tags}{tags\xspace}
\newcommand{\TagSet}{Tags\xspace}

\newcommand{\getPrincipal}{{\tt MapAttr}}
\newcommand{\appendTag}{{\tt Append}}
\newcommand{\deleteTag}{{\tt Delete}\xspace}
\newcommand{\requestTagAction}{{\tt RqstTag}}
\newcommand{\requestAttribute}{{\tt RqstAttr}}
\newcommand{\copyTag}{{\tt Copy}\xspace}
\newcommand{\modifyTag}{{\tt Modify}}
\newcommand{\resetTag}{{\tt Reset}}
\newcommand{\MboxSpecificContext}{MboxContext}
\newcommand{\Packet}{Pkt\xspace}
\newcommand{\PacketHdr}{Pkt.Hdr}
\newcommand{\PacketTag}{Pkt.\TagEnc}

\newcommand{\switch}{S}
\newcommand{\switchIndex}{k}
\newcommand{\flow}{f}
\newcommand{\flowindex}{j}
\newcommand{\chains}{C}
\newcommand{\chainIndex}{c}
\newcommand{\flows}{F}

\newcommand{\logicalmidbox}{\ensuremath{\mathit{LM}}}
\newcommand{\physicalmidbox}{\ensuremath{\mathit{PM}}}

\newcommand{\logicalmidboxindex}{\ensuremath{\mathit{m}}}
\newcommand{\nextlogicalmidboxindex}{\ensuremath{\mathit{m'}}}
\newcommand{\physicalmidboxindex}{\ensuremath{\mathit{i}}}
\newcommand{\nextphysicalmidboxindex}{\ensuremath{\mathit{i'}}}

\newcommand{\needed}{IN}
\newcommand{\obscured}{OUT}
\newcommand{\state}{s}
\newcommand{\result}{r}

\newcommand{\graph}{G}
\newcommand{\vertexSet}{V}
\newcommand{\Ingress}{\ensuremath{\mathit{In}}}
\newcommand{\Egress}{\ensuremath{\mathit{Out}}}
\newcommand{\edgeSet}{E}
\newcommand{\condition}{C}
\newcommand{\function}{f}
\newcommand{\config}{conf}
\newcommand{\packet}{\ensuremath{\mathit{pkt}}}
\newcommand{\port}{\ensuremath{\mathit{port}}}
\newcommand{\trafficClass}{TC}
\newcommand{\trafficClassIndex}{k}
\newcommand{\host}{H}
\newcommand{\trajectory}{Traj}
\newcommand{\ingress}{Ing}
\newcommand{\egress}{Egr}

\newcommand{\srcIP}{srcIP}
\newcommand{\srcPort}{srcPort}
\newcommand{\dstIP}{dstIP}
\newcommand{\dstPort}{dstPort}
\newcommand{\protocol}{protocol}

\newcommand{\transferFunction}{T}

\newcommand{\controllerTagsTable}{\ensuremath{\mathit{TagMap}}}
\newcommand{\controllerInTagsTable}{ \ensuremath{\mathit{CtrlInTagsTable}}}
\newcommand{\controllerOutTagsTable}{\ensuremath{\mathit{CtrlOutTagsTable}}}
\newcommand{\mbInTagsTable}{\ensuremath{\mathit{MBInTagsTable}}}
\newcommand{\mbOutTagsTable}{\ensuremath{\mathit{MBOutTagsTable}}}

\newcommand{\ndb}{{\tt ndb}}

\newcommand{\CPLCE}{{\em LCE}\xspace}
\newcommand{\CPLCD}{{\em LCD}\xspace}
\newcommand{\CPUniform}{{\em Rand}\xspace}
\newcommand{\CPProb}{{\em Prob}\xspace}
\newcommand{\CPPProb}{{\em PProb}\xspace}
\newcommand{\CPCentrality}{{\em Centrality}\xspace}
\newcommand{\CPHybrid}{{\em Cross}\xspace}


\newcommand{\CRLRU}{{\em LRU}\xspace}
\newcommand{\CRLFU}{{\em LFU}\xspace}
\newcommand{\CRFIFO}{{\em FIFO}\xspace}
\newcommand{\CRTTL}{{\em TTL}\xspace}
\newcommand{\CRSize}{{\em Size}\xspace}

\newcommand{\SimName}{iCache\xspace}



\newcommand{\SamePoP}{SamePoP\xspace}
\newcommand{\SameAS}{SameAS\xspace}
\newcommand{\SameISP}{SameISP\xspace}
\newcommand{\DiffISP}{DiffISP\xspace}



\newcommand{\Edge}{Edge\xspace}
\newcommand{\Core}{Core\xspace}
\newcommand{\Middle}{Middle\xspace}

\newcommand{\HE}{HE\xspace}
\newcommand{\SD}{SD\xspace}
\newcommand{\GD}{GD\xspace}
\newcommand{\JL}{JL\xspace}
\newcommand{\BJ}{BJ\xspace}
\newcommand{\SC}{SC\xspace}
\newcommand{\HA}{HA\xspace}
\newcommand{\JS}{JS\xspace}
\newcommand{\LN}{LN\xspace}
\newcommand{\ZJ}{ZJ\xspace}
\newcommand{\Tibet}{TB\xspace}
\newcommand{\JX}{JX\xspace}
\newcommand{\AH}{AH\xspace}
\newcommand{\GZ}{GZ\xspace}
\newcommand{\SH}{SH\xspace}


\newcommand{\ClientIndex}{\ensuremath{\mathit{c}}}
\newcommand{\RouterIndex}{\ensuremath{\mathit{r}}}
\newcommand{\RequestIndex}{\ensuremath{\mathit{q}}}
\newcommand{\NumRouters}{\ensuremath{\mathit{R}}}
\newcommand{\NumRequests}{\ensuremath{\mathit{V}}}
\newcommand{\RouterHits}{\ensuremath{\mathit{Hit}}}
\newcommand{\RouterMiss}{\ensuremath{\mathit{Misses}}}
\newcommand{\Bytes}{\ensuremath{\mathit{Bytes}}}

\newcommand{\scenario}{\ensuremath{\mathit{s}}}
\newcommand{\combo}{\ensuremath{\mathit{pr}}}
\newcommand{\Score}{\ensuremath{\mathit{Score}}}
\newcommand{\Perf}{\ensuremath{\mathit{Perf}}}
\newcommand{\QoE}{\ensuremath{\mathit{QoE}}}
\newcommand{\NormQoE}{\ensuremath{\mathit{NormQoE}}}

